New level of precision in study of neutron beta-decay -- Theoretical basics and experimental backgrounds

The article provides a theoretical substantiation for a significant increase in the level of accuracy in determining the neutron lifetime using an alternative concept of neutron beta decay. Neutrons are distributed among different subsets depending on the sign of the scalar product of the neutron spin vector and momentum of the emitted electron during decay. Therefore, the neutron lifetime can be determined separately for each of the subsets as the inverse frequency of its decay, which is to be averaged over the number of neutrons in this subset. The total neutron lifetime on the total set of neutrons is calculated by averaging the partial (basic) lifetimes, considering their weights. The weights of the basic lifetimes are calculated for two weighing methods, leading, respectively, to the so-called lifetime of "nonpolarized" neutrons, the weighted average lifetime of neutrons and the central lifetime, i.e. the arithmetic mean for the basic lifetimes of neutrons. The dependence between different average neutron lifetimes through the integral asymmetry parameter calculated by using known experimental data leads to simple analytical expressions. The numerical estimate of the weighted average neutron lifetime gives a value that is in good agreement with the results of well-known experiments, which proves the validity of the proposed concept of neutron beta decay. This article includes necessary conditions for a new experiment to bring the neutron lifetime determination to a new level of accuracy.

==> inx_proba.tex <==
%%
%% This file will generate fast loadable files and documentation
%% driver files from the doc files in this package when run through
%% LaTeX or TeX.
%%
%% Copyright 2007-2020 Elsevier Ltd
%%
%% This file is part of the 'Elsarticle Bundle'.
%% ---------------------------------------------
%%
%% It may be distributed under the conditions of the LaTeX Project Public
%% License, either version 1.2 of this license or (at your option) any
%% later version.  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%%
%% The list of all files belonging to the 'Elsarticle Bundle' is
%% given in the file 'manifest.txt'.
%%
%% $Id: elsarticle.ins 191 2020-11-23 11:13:24Z rishi $
%%
%%
\input docstrip.tex
%%\keepsilent

\preamble

Copyright 2007-2020 Elsevier Ltd

This file is part of the 'Elsarticle Bundle'.
-------------------------------------------

It may be distributed under the conditions of the LaTeX Project Public
License, either version 1.2 of this license or (at your option) any
later version.  The latest version of this license is in
   http://www.latex-project.org/lppl.txt
and version 1.2 or later is part of all distributions of LaTeX
version 1999/12/01 or later.

The list of all files belonging to the 'Elsarticle Bundle' is
given in the file `manifest.txt'.

\endpreamble

\askforoverwritefalse

\generate{\file{elsarticle.cls}{\from{elsarticle.dtx}{class}}}
\obeyspaces
\Msg{*************************************************************}
\Msg{*                                                           *}
\Msg{* To finish the installation you have to move the following *}
\Msg{* file into a directory searched by TeX:                    *}
\Msg{*                                                           *}
\Msg{*     elsarticle.cls                                        *}
\Msg{*         and                                               *}
\Msg{*     elsarticle-*.bst                                      *}
\Msg{*                                                           *}
\Msg{* To produce the documentation go to the ../contrib folder  *}
\Msg{* and run the file elsdoc.tex through pdfLaTeX              *}
\Msg{* or use the Makefile which is far more easier.             *}
\Msg{*                                                           *}
\Msg{* Happy TeXing!                                             *}
\Msg{*                                                           *}
\Msg{*************************************************************}

\endbatchfile
